Comparing Generative Chatbots Based on Process Requirements

Business processes are commonly represented by modelling languages, such as Event-driven Process Chain (EPC), Yet Another Workflow Language (YAWL), and the most popular standard notation for modelling business processes, the Business Process Model and Notation (BPMN). Most recently, chatbots, programs that allow users to interact with a machine using natural language, have been increasingly used for business process execution support. A recent category of chatbots worth mentioning is generative-based chatbots, powered by Large Language Models (LLMs) such as OpenAI's Generative Pre-Trained Transformer (GPT) model and Google's Pathways Language Model (PaLM), which are trained on billions of parameters and support conversational intelligence. However, it is not clear whether generative-based chatbots are able to understand and meet the requirements of constructs such as those provided by BPMN for process execution support. This paper presents a case study to compare the performance of prominent generative models, GPT and PaLM, in the context of process execution support. The research sheds light into the challenging problem of using conversational approaches supported by generative chatbots as a means to understand process-aware modelling notations and support users to execute their tasks.

==> old/paper_extension.tex <==
**Spotlight on Research Paper: "Integrating Large Language Models into Multiagent Systems for Enhanced Self-Adaptation"**

In the complex world of autonomic computing, self-adaptation is essential for managing multiagent systems (MASs). These systems require sophisticated, direct communication to enhance cooperation, reduce coordination challenges, and adapt dynamically. Our latest research provides an innovative approach, propelling the field further by integrating Large Language Models (LLMs) like GPT-4 into MASs, grounded on the robust MAPE-K model.

In our research, we offer a new paradigm for MAS self-adaptation of autonomous systems leveraging LLM capabilities. This idea presents a significant shift away from traditional models where agents evolve their communication systems over time. We explore the potential of equipping autonomous agents with LLMs from inception and hypothesize a remarkable enhancement in agents' abilities to execute complex tasks and adapt using advanced communication systems.

Our innovative architecture embeds GPT-4, a cutting-edge LLM, within each agent of the MAS. In doing so, we create an environment where every autonomous entity communicates and self-adapts using natural language processing. This methodology, extended from the MAPE-K model, allows for adaptivity in dynamically changing environments, giving our agents advanced communicative capabilities and a unique ability to intelligently react to evolving situations.

To validate our approach, we used a simplified marketplace scenario as a testbed, where autonomous agents, each equipped with an embedded LLM, are tasked with buying and selling books. These agents demonstrated decision-making and emergent behavior, underscoring the potential for self-adaptation.

While the integration of LLMs into MASs presents substantial challenges, such as computational overheads and ethical considerations, we believe it's a promising venture. The use of LLMs in multiagent systems could revolutionize how agents understand, learn from, and interact with their environment and other agents, paving the way for more robust, sophisticated communication, improved adaptability, and enhanced problem-solving capabilities.
